A Provably Effective Method for Pruning Experts in Fine-tuned Sparse Mixture-of-Experts

The sparsely gated mixture of experts (MoE) architecture sends different inputs to different subnetworks, i.e., experts, through trainable routers. MoE reduces the training computation significantly for large models, but its deployment can be still memory or computation expensive for some downstream tasks. Model pruning is a popular approach to reduce inference computation, but its application in MoE architecture is largely unexplored. To the best of our knowledge, this paper provides the first provably efficient technique for pruning experts in finetuned MoE models. We theoretically prove that prioritizing the pruning of the experts with a smaller change of the routers l2 norm from the pretrained model guarantees the preservation of test accuracy, while significantly reducing the model size and the computational requirements. Although our theoretical analysis is centered on binary classification tasks on simplified MoE architecture, our expert pruning method is verified on large vision MoE models such as VMoE and E3MoE finetuned on benchmark datasets such as CIFAR10, CIFAR100, and ImageNet.

==> experiments.tex <==
\section{Experimental Results}\label{experiments}

We implement the proposed \textit{change in router's $l_2$ norm} based expert pruning method in state-of-the-art vision MoE models fine-tuned on several benchmark datasets such as CIFAR-10, CIFAR-100 \citep{krizhevsky2009learning} and ImageNet \citep{russakovsky2015imagenet}. More specifically, we implement the method to prune the 
released fine-tuned sparse vision MoE (V-MoE) by \citet{riquelme2021scaling}. Moreover, we present results on the released fine-tuned efficient ensembles of experts in MoE ($\text{E}^3$-MoE) by \citet{allingham2022sparse}.

\subsection{The Pruned Models}
\textbf{The V-MoE models}. The released set of V-MoE models by \citet{riquelme2021scaling} includes the pre-trained version of the models on ImageNet-21k \citep{kolesnikov2020big} and the two fine-tuned versions on CIFAR-10 and ImageNet-1k (i.e., ILSVRC2012), respectively. The models contain 12 transformer encoders (encoders 0, 1, ..., and 11). Every odd encoder (i.e., encoders 1, 3, 5, 7, 9, and 11) is the MoE encoder. Each MoE encoder contains $8$ experts (i.e., $k=8$). The input images are divided into $16\times 16$ patches and then transformed into the encoder's hidden dimension of $768$ (i.e., $d=768$). The MoE hidden dimension is $3072$ (i.e., $m=3072$). The CIFAR-10 fine-tuned version contains 65 tokens for an input image (i.e., $n=65$). The ImageNet fine-tuned version contains 577 tokens for an input image (i.e., $n=577$). The MoE routers in the model implement token-choice routing where each token is routed to 2 experts (i.e., $l=2$). The total number of parameters in the model is roughly 979 million. SGD with momentum and cosine learning rate decay is implemented to obtain the fine-tuned models. The fine-tuning steps are 1000 and 10,000 for CIFAR-10 and ImageNet, respectively. More details can be found in \citet{riquelme2021scaling}.

\textbf{The $\text{E}^3$-MoE models}. \citet{allingham2022sparse} proposed the efficient ensembles of experts in MoE (i.e., $\text{E}^3$-MoE) to improve the generalization performance of V-MoE. The architecture implements the ensembles of experts where, in each MoE encoder the experts are divided into multiple ensembles. The released set of $\text{E}^3$-MoE models includes the pre-trained version on ImageNet and the fine-tuned version on CIFAR-100. The models contain 8 transformer encoders (i.e., encoders 0, 1, ..., and 7), where the last two encoders contain the ensemble of MoEs (i.e., encoders 5 and 7). There are 2 MoE ensembles in the model and each MoE ensembles contains 4 experts per MoE encoder (i.e., $k=4$). The input images are divided into $32\times 32$ patches and then transformed into encoder's hidden dimension of 512 (i.e., $d=512$) where the MoE hidden dimension is 2048 (i.e., $m=2048$). The number of tokens per image in each encoder is $65$ (i.e., $n=65$). The MoE routers implement the token-choice routing, selecting one expert per token (i.e., $l=1$). Total number of parameters in the model is roughly 167 million. Again, SGD with momentum and cosine learning rate decay is implemented during fine-tuning for 2000 steps.

\textbf{Pruning and post-pruning fine-tuning details}. We use both the pre-trained and the fine-tuned versions of the released model to calculate the change in the router's norm for each expert. We apply our pruning method over each MoE layer separately in V-MoE model while applying the method separately over the experts in each ensemble group of each MoE encoder in the $\text{E}^3$-MoE model. We implement the pruned model in parallel into two NVIDIA RTX A5000 GPUs for inference and the post-pruning fine-tuning. For post-pruning fine-tuning, as the model size is large, we divide the batch size into half from the original case for CIFAR-10 and CIFAR-100. However, the number of steps is the same. For the same reason, we divide the original batch-size by 32 folds so as the learning rate for ImageNet and hence increase the post-training fine-tuning steps by 32 times of the original. Rest of the hyperparameters are same as in the original fine-tuning process described by the authors.

\subsection{Results}
\textbf{Generalization performance}. Primarily, we verify the effectiveness of our method compared to the random pruning baseline. As shown in Figure \ref{cifar_10_random} for CIFAR-10, our method can effectively select the task-specific experts as it retains the original performance while random pruning of experts falls sharply after a small pruning ratio\footnote{Note that, in all of the results in this section, the pruning ratio is calculated over the parameters of the whole model, not over the parameters of the MoE encoder only}. Figure \ref{cifar_10_only_pruned} presents generalization results on CIFAR-10 without post-pruning fine-tuning. As we can see, the method can prune 50\% of the experts (35\% of the whole model) while maintaining accuracy within 1\% of the unpruned model when we do not prune from the penultimate MoE layer (i.e., encoder 9 for V-MoE). However, as described in \citet{riquelme2021scaling}, due to the extra sensitivity of the penultimate MoE layer, pruning in the layer is not feasible without post-pruning fine-tuning. However, as shown in Figure \ref{cifar_10_pruned_finetuned}, we can overcome the limitation by post-pruning fine-tuning and prune up to the maximum possible percentage (75\% of the experts, 60\% of the whole model)\footnote{pruning more than 6 experts out of 8 experts is not allowed for $l=2$.}.
\begin{figure}[ht]
%\vspace{-2mm}
    \begin{subfigure}[(b)]{0.48\linewidth}
        \centering
        \includegraphics[width=0.99\linewidth]{Fig/cifar_10_proposed_vs_random_only_pruned.png}
        %\vspace{-4mm}
        \caption{}
        \label{cifar_10_random}
    \end{subfigure}
    \hfill
    \begin{subfigure}[(a)]{0.49\linewidth}
        \centering
        \includegraphics[width=0.99\linewidth]{Fig/cifar_10_only_pruned_acc.png}
        %\vspace{-4mm}
        \caption{}
        \label{cifar_10_only_pruned}
    \end{subfigure}
    %\vspace{-3mm}
    \caption{Generalization performance of the pruned V-MoE on CIFAR-10: (a) Comparison to random pruning, (b) with and without pruning in encoder 9}
    \vspace{-1mm}
\end{figure}

We found similar results for pruning $\text{E}^3$-MoE on CIFAR-100 (75\% of the experts; 45\% of the whole model) and pruning V-MoE on ImageNet (42\% of the experts; 35\% of whole model). The results are presented in Figure \ref{cifar_100_only_pruned}, Figure \ref{cifar_100_pruned_finetuned} and Figure \ref{imagenet_only_pruned}, Figure \ref{imagenet_pruned_fine_tuned}, respectively. As we can see, when the size of the downstream task goes up (1000 class classification in ImageNet compared to 100 class classification in CIFAR-100 and 10 class classification in CIFAR-10) the maximum allowable pruning ratio goes down as more experts are now important for the larger sized task.
\begin{figure}[ht]
%\vspace{-2mm}
    \begin{subfigure}[(a)]{0.49\linewidth}
        \centering
        \includegraphics[width=0.99\linewidth]{Fig/cifar_100_only_pruned_acc.png}
        %\vspace{-4mm}
        \caption{}
        \label{cifar_100_only_pruned}
    \end{subfigure}
    \hfill
    \begin{subfigure}[(b)]{0.48\linewidth}
        \centering
        \includegraphics[width=0.99\linewidth]{Fig/cifar_100_pruned_finetuned_acc.png}
        %\vspace{-4mm}
        \caption{}
        \label{cifar_100_pruned_finetuned}
    \end{subfigure}
    %\vspace{-3mm}
    \caption{Generalization performance of the pruned $\text{E}^3$-MoE on CIFAR-100: (a) without post-pruning fine-tuning, (b) with post-pruning fine-tuning}
    \vspace{-3mm}
\end{figure}
\begin{figure}[ht]
%\vspace{-2mm}
    \begin{subfigure}[(a)]{0.49\linewidth}
        \centering
        \includegraphics[width=0.99\linewidth]{Fig/imagenet_only_pruned_acc.png}
        %\vspace{-4mm}
        \caption{}
        \label{imagenet_only_pruned}
    \end{subfigure}
    \hfill
    \begin{subfigure}[(b)]{0.48\linewidth}
        \centering
        \includegraphics[width=0.99\linewidth]{Fig/imagenet_pruned_finetuned_acc.png}
        %\vspace{-4mm}
        \caption{}
        \label{imagenet_pruned_fine_tuned}
    \end{subfigure}
    %\vspace{-3mm}
    \caption{Generalization performance of the pruned V-MoE on ImageNet: (a) without post-pruning fine-tuning, (b) with post-pruning fine-tuning}
    \vspace{-3mm}
\end{figure}

\textbf{Inference efficiency}. We measure the inference efficiency of the pruned model in terms of FLOPs per image and the inference time. Figure \ref{cifar_10_flop} shows the linear reduction of inference FLOPs per image with the increment of pruning ratio in pruning V-MoE on CIFAR-10. Furthermore, Figure \ref{cifar_10_time} shows the linear reduction of inference time with the increment of pruning ratio for the setting. By combining these two results with the results in Figure \ref{cifar_10_pruned_finetuned} we can infer that the proposed pruning method can reduce 40\% of the inference FLOPs and 40\% of the inference time. Moreover, the linear reduction of FLOPs and time indicates the prompt implementation of the method without any loss of estimated efficiency (e.g., due to the overhead of the dedicated software kernels or hardware) as our results are generated from the computation on typical modern GPUs without any requirement of special software (e.g., dedicated CUDA kernels).     
\begin{figure}[ht]
%\vspace{-2mm}
    \begin{subfigure}[(a)]{0.49\linewidth}
        \centering
        \includegraphics[width=0.99\linewidth]{Fig/cifar_10_gflop.png}
        %\vspace{-4mm}
        \caption{}
        \label{cifar_10_flop}
    \end{subfigure}
    \hfill
    \begin{subfigure}[(b)]{0.48\linewidth}
        \centering
        \includegraphics[width=0.99\linewidth]{Fig/cifar_10_time.png}
        %\vspace{-4mm}
        \caption{}
        \label{cifar_10_time}
    \end{subfigure}
    %\vspace{-3mm}
    \caption{Inference cost of the pruned V-MoE model on CIFAR-10 in terms of: (a) FLOPs per image, (b) Inference time on the whole test}
    \vspace{-3mm}
\end{figure}

We have similar results for pruning $\text{E}^3$-MoE on CIFAR-100 (15\% reduction of FLOPs, 15\% reduction of time) and pruning V-MoE on ImageNet (14\% reduction of FLOPs, 14\% reduction of time). The results are presented in Figure \ref{cifar_100_flop}, \ref{cifar_100_time} and Figure \ref{imagenet_flop}, \ref{imagenet_time}, respectively. The slight sublinearity in Figure \ref{cifar_100_time} occurs from the parallel implementation of ensembles. The relatively less reduction of FLOPs and time in CIFAR-100 compared to CIFAR-10 occurs from the fact that the unpruned $\text{E}^3$-MoE is much smaller than the unpruned V-MoE in terms of parameters (167 million compared to 979 million).
\begin{figure}[ht]
%\vspace{-2mm}
    \begin{subfigure}[(a)]{0.49\linewidth}
        \centering
        \includegraphics[width=0.99\linewidth]{Fig/cifar_100_gflop.png}
        %\vspace{-4mm}
        \caption{}
        \label{cifar_100_flop}
    \end{subfigure}
    \hfill
    \begin{subfigure}[(b)]{0.48\linewidth}
        \centering
        \includegraphics[width=0.99\linewidth]{Fig/cifar_100_time.png}
        %\vspace{-4mm}
        \caption{}
        \label{cifar_100_time}
    \end{subfigure}
    %\vspace{-3mm}
    \caption{Inference cost of the pruned $\text{E}^3$-MoE model on CIFAR-100 in terms of: (a) FLOPs per image, (b) Inference time on the whole test}
    \vspace{-3mm}
\end{figure}
\begin{figure}[ht]
%\vspace{-2mm}
    \begin{subfigure}[(a)]{0.49\linewidth}
        \centering
        \includegraphics[width=0.99\linewidth]{Fig/imagenet_gflop.png}
        %\vspace{-4mm}
        \caption{}
        \label{imagenet_flop}
    \end{subfigure}
    \hfill
    \begin{subfigure}[(b)]{0.48\linewidth}
        \centering
        \includegraphics[width=0.99\linewidth]{Fig/imagenet_time.png}
        %\vspace{-4mm}
        \caption{}
        \label{imagenet_time}
    \end{subfigure}
    %\vspace{-3mm}
    \caption{Inference cost of the pruned V-MoE model on ImageNet in terms of: (a) FLOPs per image, (b) Inference time on the whole test}
    \vspace{-3mm}
\end{figure}
